MAD Speech: Measures of Acoustic Diversity of Speech

Generative spoken language models produce speech in a wide range of voices, prosody, and recording conditions, seemingly approaching the diversity of natural speech. However, the extent to which generated speech is acoustically diverse remains unclear due to a lack of appropriate metrics. We address this gap by developing lightweight metrics of acoustic diversity, which we collectively refer to as MAD Speech. We focus on measuring five facets of acoustic diversity: voice, gender, emotion, accent, and background noise. We construct the metrics as a composition of specialized, per-facet embedding models and an aggregation function that measures diversity within the embedding space. Next, we build a series of datasets with a priori known diversity preferences for each facet. Using these datasets, we demonstrate that our proposed metrics achieve a stronger agreement with the ground-truth diversity than baselines. Finally, we showcase the applicability of our proposed metrics across several real-life evaluation scenarios. MAD Speech is made publicly accessible.

==> tables/accent_main.tex <==
\begin{table*}[ht]
\centering
\resizebox{\linewidth}{!}{\begin{tabular}{lccccc}
\toprule
                                                \multicolumn{6}{c}{Accent} \\
\midrule
                                                   &  Avg. Cosine &     Vendi score &   Token entropy & Distinct n-grams &       self-BLEU \\ \midrule
                                                   
Soundstream raw avg. over time & 0.234 (± 0.517) & 0.217 (± 0.581) &      -           &         -              &         -        \\

Soundstream raw max. over time & 0.342 (± 0.418) & 0.023 (± 0.518) &       -           &         -              &         -    \\
 
Speech Sim & 0.446 (± 0.476) & 0.574 (± 0.328) &         -           &         -              &         -          \\

Trained from scratch & \underline{0.995} (± 0.016) & \textbf{1.000} (± 0.000) &          -           &         -              &         -  \\

Wav2vec-BERT raw avg. over time & 0.425 (± 0.415) & 0.557 (± 0.376) &        -           &         -              &         -           \\

Wav2vec-BERT raw max. over time & 0.443 (± 0.407) & 0.369 (± 0.394) &     -           &         -              &         -         \\

HuBERT raw avg. over time & 0.372 (± 0.425) & 0.526 (± 0.366) &        -           &         -              &         -      \\

HuBERT raw max. over time & 0.346 (± 0.393) & 0.286 (± 0.385) &       -           &         -              &         -         \\

MADSpeech accent proj. & 0.991 (± 0.021) & \textbf{1.000} (± 0.000) &         -           &         -              &         -           \\ \midrule

Soundstream tokens RVQ-level 0 &         -        &        -         & 0.230 (± 0.565) &       0.127 (± 0.614) & 0.035 (± 0.609) \\

Wav2vec-BERT tokens - vocab. size 256 &            -        &        -         & 0.246 (± 0.529) &       0.189 (± 0.568) & 0.033 (± 0.580) \\
                            
Wav2vec-BERT tokens - vocab. size 512 &          -        &        -        & 0.258 (± 0.554) &       0.207 (± 0.573) & 0.092 (± 0.564) \\
                           
Wav2vec-BERT tokens - vocab. size 1024 &          -        &        -       & 0.318 (± 0.510) &       0.211 (± 0.552) & 0.085 (± 0.539) \\
                           
Wav2vec-BERT tokens - vocab. size 4096 &          -        &        -        & 0.315 (± 0.534) &       0.196 (± 0.553) & 0.105 (± 0.553) \\
                               
HuBERT tokens - vocab size 50 &          -        &        -        & 0.165 (± 0.586) &       0.080 (± 0.557) & 0.043 (± 0.576) \\

HuBERT tokens - vocab size 100 &        -        &        -     & 0.190 (± 0.582) &       0.130 (± 0.553) & 0.098 (± 0.545) \\

HuBERT tokens - vocab size 200 &         -        &        -      & 0.142 (± 0.586) &       0.134 (± 0.544) & 0.071 (± 0.551) \\
\bottomrule
\end{tabular}}
\caption{Accent experiment. Average Spearman correlation ($\pm$ standard error) between the class entropy in VCTK and diversity scores induced by speech representations. Best results are in bold, second best results are underlined.}
\label{tab:accent-tab}
\end{table*}


==> tables/background_noise.tex <==
\begin{table*}[ht]
\centering
\resizebox{\linewidth}{!}{\begin{tabular}{lccccc}
\toprule
                                                 \multicolumn{6}{c}{ Background Noise} \\
\midrule

&            \multicolumn{5}{c}{standard}     \\ \cmidrule(lr){2-6}
                                                   &    Avg. Cosine &       Vendi score &    Token entropy &   Distinct n-grams &          self-BLEU  \\ \midrule
                                                   
 Soundstream raw avg. over time &   \hphantom{-}0.141 (± 0.390) &   \hphantom{-}0.265 (± 0.433) &     \multicolumn{1}{c}{-}            &          \multicolumn{1}{c}{-}              &       \multicolumn{1}{c}{-}              \\

 Soundstream raw max. over time &  \hphantom{-}0.149 (± 0.380) &  \hphantom{-}0.199 (± 0.476) &        \multicolumn{1}{c}{-}         &         \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}        \\
                                 
 Speech Sim &  \hphantom{-}0.254 (± 0.309) &  \hphantom{-}0.466 (± 0.322) &          \multicolumn{1}{c}{-}         &         \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}           \\
                                          
 Trained from scratch &  \hphantom{-}0.173 (± 0.355) &   \hphantom{-}0.355 (± 0.404) &       \multicolumn{1}{c}{-}         &         \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}       \\
                                      
 Wav2vec-BERT raw avg. over time &  -0.014 (± 0.417) &  -0.070 (± 0.452) &       \multicolumn{1}{c}{-}         &         \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}        \\
                                      
 Wav2vec-BERT raw max. over time &  \hphantom{-}0.013 (± 0.385) &  \hphantom{-}0.136 (± 0.448) &      \multicolumn{1}{c}{-}         &         \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}       \\
                                      
 HuBERT raw avg. over time &  \hphantom{-}0.218 (± 0.356) &  \hphantom{-}\textbf{0.531} (± 0.332) &      \multicolumn{1}{c}{-}         &         \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}         \\
                                    
 HuBERT raw max. over time &  \hphantom{-}0.043 (± 0.386) &  -0.155 (± 0.508) &      \multicolumn{1}{c}{-}         &         \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}        \\
                                    
 MADSpeech background noise proj. &  \hphantom{-}0.116 (± 0.359) &  \hphantom{-}\underline{0.469} (± 0.413) &       \multicolumn{1}{c}{-}         &         \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}         \\ \midrule


 Soundstream tokens RVQ-level 0 &   \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}       &  \hphantom{-}0.390 (± 0.446) &       \hphantom{-}0.136 (± 0.449) &  -0.020 (± 0.426)\\

 Wav2vec-BERT tokens - vocab. size 256 &  \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}      &  \hphantom{-}0.027 (± 0.430) &        \hphantom{-}0.058 (± 0.445) &  -0.039 (± 0.413) \\

 Wav2vec-BERT tokens - vocab. size 512 &   \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}      &  \hphantom{-}0.151 (± 0.408) &        \hphantom{-}0.081 (± 0.429) &  -0.062 (± 0.450) \\

 Wav2vec-BERT tokens - vocab. size 1024 &   \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}        &  \hphantom{-}0.123 (± 0.446) &        \hphantom{-}0.067 (± 0.447) &   \hphantom{-}0.020 (± 0.393) \\

 Wav2vec-BERT tokens - vocab. size 4096  &  \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}      &  \hphantom{-}0.117 (± 0.450) &        \hphantom{-}0.019 (± 0.428) &  \hphantom{-}0.025 (± 0.444)  \\

 HuBERT tokens - vocab size 50 &  \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}       &  \hphantom{-}0.285 (± 0.491) &        \hphantom{-}0.102 (± 0.455) &  \hphantom{-}0.050 (± 0.428)  \\

 HuBERT tokens - vocab size 100 &  \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}       &  \hphantom{-}0.298 (± 0.463) &      -0.015 (± 0.494) &  \hphantom{-}0.085 (± 0.425) \\

 HuBERT tokens - vocab size 200 &    \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}       &  \hphantom{-}0.337 (± 0.450) &        \hphantom{-}0.102 (± 0.455) &  \hphantom{-}0.070 (± 0.445)  \\



\midrule
\midrule

&            \multicolumn{5}{c}{w/ no background noise class}     \\ \cmidrule(lr){2-6}
                                                   &    Avg. Cosine &       Vendi score &    Token entropy &   Distinct n-grams &          self-BLEU  \\ \midrule


 Soundstream raw avg. over time &   -0.237 (± 0.145) &  -0.974 (± 0.032) &          \multicolumn{1}{c}{-}         &         \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}           \\

 Soundstream raw max. over time &  -0.164 (± 0.139) & -0.097 (± 0.062) &         \multicolumn{1}{c}{-}         &         \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}         \\
                                 
 Speech Sim &    -0.303 (± 0.232) &  -0.727 (± 0.212) &          \multicolumn{1}{c}{-}         &         \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}      \\
                                          
 Trained from scratch &  \hphantom{-}0.319 (± 0.267) &  \hphantom{-}\underline{0.665} (± 0.277) &        \multicolumn{1}{c}{-}         &         \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}      \\
                                      
 Wav2vec-BERT raw avg. over time &  -0.037 (± 0.129) &  -0.928 (± 0.032) &        \multicolumn{1}{c}{-}         &         \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}      \\
                                      
 Wav2vec-BERT raw max. over time &  \hphantom{-}0.298 (± 0.145) &  -0.084 (± 0.066) &       \multicolumn{1}{c}{-}         &         \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}       \\
                                      
 HuBERT raw avg. over time &  -0.009 (± 0.302) &  -0.849 (± 0.117) &      \multicolumn{1}{c}{-}         &         \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}     \\
                                    
 HuBERT raw max. over time &  -0.129 (± 0.354) &  \hphantom{-}0.585 (± 0.298) &        \multicolumn{1}{c}{-}         &         \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}      \\
                                    
 MADSpeech background noise proj. &  \hphantom{-}0.314 (± 0.279) &  \hphantom{-}\textbf{0.738} (± 0.212) &        \multicolumn{1}{c}{-}         &         \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}         \\ \midrule


 Soundstream tokens RVQ-level 0 &    \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}        &  -0.897 (± 0.104) &       -0.961 (± 0.046) &  -0.214 (± 0.128) \\

 Wav2vec-BERT tokens - vocab. size 256 &   \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}       &  -0.920 (± 0.091) &      -0.955 (± 0.060) &  -0.210 (± 0.135) \\

 Wav2vec-BERT tokens - vocab. size 512 &   \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}        &  -0.925 (± 0.081) &      -0.967 (± 0.046) &  -0.206 (± 0.130) \\

 Wav2vec-BERT tokens - vocab. size 1024 &     \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}       &  -0.971 (± 0.036) &      -0.975 (± 0.029) &  -0.211 (± 0.130) \\

 Wav2vec-BERT tokens - vocab. size 4096  &  \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}      &  -0.935 (± 0.069) &      -0.974 (± 0.030) &  -0.219 (± 0.132) \\

 HuBERT tokens - vocab size 50 &   \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}       &  \hphantom{-}0.439 (± 0.308) &       \hphantom{-}0.449 (± 0.315) &  \hphantom{-}0.317 (± 0.343) \\

 HuBERT tokens - vocab size 100 &  \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}        &  \hphantom{-}0.445 (± 0.304) &       \hphantom{-}0.435 (± 0.327) &   \hphantom{-}0.348 (± 0.320) \\

 HuBERT tokens - vocab size 200 &   \multicolumn{1}{c}{-}               &        \multicolumn{1}{c}{-}        &  \hphantom{-}0.426 (± 0.294) &       \hphantom{-}0.388 (± 0.324) &  \hphantom{-}0.307 (± 0.348) \\ \bottomrule
\end{tabular}}
\caption{Caption}
\label{tab:background-noise-tab}
\end{table*}


==> tables/emotion_main.tex <==
\begin{table*}[ht]
\renewcommand{\arraystretch}{.5}
\centering
\resizebox{\linewidth}{!}{\begin{tabular}{lcccccccccc}
\toprule[\heavyrulewidth] \\
                                               \multicolumn{11}{c}{\Huge Emotion} \\[.2cm]
\midrule[\heavyrulewidth]
                                                   &            \multicolumn{5}{c}{\Huge EmoV} &    \multicolumn{5}{c}{\Huge Expresso}     \\ \cmidrule(lr){2-6} \cmidrule(lr){7-11}
                                                   &  \Huge Avg. Cosine &      \Huge Vendi score &   \Huge Token entropy & \Huge Distinct n-grams &       \Huge self-BLEU &  \Huge Avg. Cosine &     \Huge Vendi score &    \Huge Token entropy & \Huge Distinct n-grams &        \Huge self-BLEU \\ \midrule[\heavyrulewidth] \\
                                                   
\Huge Soundstream raw avg. over time & \Huge \hphantom{-}0.137 (± 0.573) & \Huge \hphantom{-}0.714 (± 0.250) &         \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}          & \Huge \hphantom{-}0.357 (± 0.383) & \Huge \hphantom{-}0.495 (± 0.348) &                    \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}              \\[.3cm]

\Huge Soundstream raw max. over time & \Huge \hphantom{-}0.008 (± 0.392) & \Huge \hphantom{-}0.098 (± 0.454) &         \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}         & \Huge \hphantom{-}0.239 (± 0.352) & \Huge \hphantom{-}0.105 (± 0.469) &     \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}         \\[.3cm]
                              
\Huge Speech Sim & \Huge \hphantom{-}0.809 (± 0.200) & \Huge \hphantom{-}0.823 (± 0.193) &     \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}         & \Huge \hphantom{-}0.739 (± 0.249) & \Huge \hphantom{-}0.864 (± 0.128) &      \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}         \\[.3cm]

\Huge Trained from scratch & \Huge \hphantom{-}0.991 (± 0.020) & \Huge \hphantom{-}0.962 (± 0.051) &     \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}        & \Huge \hphantom{-}\underline{0.998} (± 0.008) & \Huge \hphantom{-}0.988 (± 0.018) &     \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}        \\[.3cm]

\Huge Wav2vec-BERT raw avg. over time & \Huge \hphantom{-}0.682 (± 0.182) & \Huge \hphantom{-}0.594 (± 0.080) &    \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}        & \Huge \hphantom{-}0.668 (± 0.170) & \Huge \hphantom{-}0.705 (± 0.070) &     \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}        \\[.3cm]

\Huge Wav2vec-BERT raw max. over time & \Huge \hphantom{-}0.502 (± 0.188) & \Huge \hphantom{-}0.417 (± 0.227) &     \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}        & \Huge \hphantom{-}0.538 (± 0.214) & \Huge \hphantom{-}0.534 (± 0.251) &     \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}        \\[.3cm]

\Huge HuBERT raw avg. over time & \Huge \hphantom{-}0.785 (± 0.148) & \Huge \hphantom{-}0.683 (± 0.088) &     \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}         & \Huge \hphantom{-}0.725 (± 0.154) & \Huge \hphantom{-}0.725 (± 0.064) &     \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}         \\[.3cm]

\Huge HuBERT raw max. over time & \Huge \hphantom{-}0.209 (± 0.330) & \Huge -0.041 (± 0.385) &     \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}        & \Huge \hphantom{-}0.243 (± 0.358) & \Huge \hphantom{-}0.172 (± 0.387) &      \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}        \\[.3cm]
                                    
\Huge MADSpeech emotion proj. & \Huge \hphantom{-}\textbf{0.995} (± 0.016) &  \Huge \Huge \hphantom{-}\underline{0.993} (± 0.019) &    \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}       & \Huge \hphantom{-}\textbf{0.999} (± 0.007) & \Huge \hphantom{-}0.987 (± 0.017) &    \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}        \\[.3cm] \midrule[\heavyrulewidth] \\


\Huge Soundstream tokens RVQ-level 0 &  \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}   & \Huge \hphantom{-}0.322 (± 0.404) &     \Huge  \hphantom{-}0.401 (± 0.429) & \Huge \hphantom{-}0.299 (± 0.426) &   \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}     & \Huge \Huge \hphantom{-}0.671 (± 0.314) &    \Huge   \hphantom{-}0.503 (± 0.290) &  \Huge \hphantom{-}0.591 (± 0.259) \\[.3cm]

\Huge Wav2vec-BERT tokens - vocab. size 256 &   \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}   & \Huge \Huge\hphantom{-}0.709 (± 0.222) &    \Huge  \hphantom{-}0.286 (± 0.515) & \Huge \hphantom{-}0.297 (± 0.484) &   \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}   & \Huge  \hphantom{-}0.158 (± 0.441) &  \Huge     -0.002 (± 0.521) & \Huge -0.062 (± 0.459) \\[.3cm]

\Huge Wav2vec-BERT tokens - vocab. size 512 &   \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}    & \Huge \hphantom{-}0.697 (± 0.230) &     \Huge  \hphantom{-}0.349 (± 0.500) & \Huge \hphantom{-}0.294 (± 0.458) &   \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}  & \Huge  \hphantom{-}0.209 (± 0.410) &    \Huge  -0.050 (± 0.488) & \Huge -0.133 (± 0.440) \\[.3cm]

\Huge Wav2vec-BERT tokens - vocab. size 1024 &   \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}   & \Huge \hphantom{-}0.663 (± 0.287) &    \Huge   \hphantom{-}0.406 (± 0.510) & \Huge \hphantom{-}0.341 (± 0.467) &   \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}   & \Huge -0.005 (± 0.468) &    \Huge  -0.109 (± 0.497) &  \Huge -0.269 (± 0.457) \\[.3cm]

\Huge Wav2vec-BERT tokens - vocab. size 4096 &  \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -} & \Huge \hphantom{-}0.378 (± 0.431) &   \Huge    \hphantom{-}0.292 (± 0.524) & \Huge \hphantom{-}0.335 (± 0.475) &  \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}   & \Huge -0.020 (± 0.511) &   \Huge   -0.149 (± 0.489) & \Huge -0.409 (± 0.416) \\[.3cm]

\Huge HuBERT tokens - vocab size 50 &  \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}  & \Huge \hphantom{-}0.502 (± 0.419) &   \Huge    \hphantom{-}0.240 (± 0.514) & \Huge \hphantom{-}0.243 (± 0.481) &   \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}   & \Huge \hphantom{-}0.364 (± 0.450) &   \Huge   -0.068 (± 0.488) & \Huge \hphantom{-}0.319 (± 0.391) \\[.3cm]

\Huge HuBERT tokens - vocab size 100 &   \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}  & \Huge \hphantom{-}0.665 (± 0.326) &    \Huge   \hphantom{-}0.223 (± 0.517) & \Huge \hphantom{-}0.333 (± 0.474) &  \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}   &  \Huge \hphantom{-}0.476 (± 0.351) &    \Huge   \hphantom{-}0.036 (± 0.520) &   \Huge \hphantom{-}0.364 (± 0.389) \\[.3cm]

\Huge HuBERT tokens - vocab size 200 &  \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}  & \Huge \hphantom{-}0.742 (± 0.213) &    \Huge   \hphantom{-}0.223 (± 0.542) & \Huge \hphantom{-}0.350 (± 0.452) &   \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}     & \Huge \hphantom{-}0.623 (± 0.283) &   \Huge    \hphantom{-}0.022 (± 0.533) &   \Huge \hphantom{-}0.348 (± 0.434) \\[.3cm]
\bottomrule[\heavyrulewidth]
\end{tabular}
}
\caption{Results for emotion experiments. Average spearman correlations (and standard errors) between the variation of entropy over classes in EmoV and Expresso and different combination of speech representations and metrics. Best results are highlighted in bold, second best results are underlined.}
\label{tab:emotion-tab}
\end{table*}


==> tables/gender_speakers_main.tex <==
\begin{table*}[ht]
\renewcommand{\arraystretch}{.5}
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{lllllllllll}
\toprule[\heavyrulewidth] \\
\multicolumn{11}{c}{\Huge Gender}  \\[.2cm] \midrule[\heavyrulewidth] \\
  &     \multicolumn{2}{c}{\Huge Avg. Cosine}                  &        \multicolumn{2}{c}{\Huge Vendi score} & \multicolumn{2}{c}{\Huge Token entropy}                  & \multicolumn{2}{c}{\Huge Distinct n-grams} & \multicolumn{2}{c}{\Huge self-BLEU} \\ [.2cm] \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \\
                                                   
                                                 &         \Huge      Male &    \Huge       Female &       \Huge        Male &      \Huge     Female &       \Huge\Huge        Male &      \Huge    Female &         \Huge         Male &     \Huge      Female &       \Huge        Male &        \Huge   Female \\[.2cm] \midrule[\heavyrulewidth] \\
\Huge Soundstream raw avg. over time &    \Huge \hphantom{-}0.095 (± 0.463) & \Huge \hphantom{-}0.117 (± 0.410) & \Huge  \hphantom{-}0.092 (± 0.435)  & \Huge  \hphantom{-}0.097 (± 0.367) &       \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}             &            \multicolumn{1}{c}{\Huge -}      &            \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}          \\[.3cm]

\Huge Soundstream raw max. over time &  \Huge  \hphantom{-}0.085 (± 0.471) & \Huge -0.044 (± 0.438) & \Huge  \hphantom{-}0.109 (± 0.419)  & \Huge -0.123 (± 0.422) &             \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}             &            \multicolumn{1}{c}{\Huge -}      &            \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}     \\[.3cm]

                                          \Huge Speech Sim &  \Huge \hphantom{-}0.186 (± 0.473)  & \Huge \hphantom{-}0.129 (± 0.438) & \Huge  \hphantom{-}0.132 (± 0.440)  &  \Huge \hphantom{-}0.162 (± 0.455) &                \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}             &            \multicolumn{1}{c}{\Huge -}      &            \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}     \\[.3cm]
                                          
                                    \Huge  Trained from scratch &  \Huge \hphantom{-}\underline{0.861} (± 0.076)  &  \Huge \hphantom{-}\underline{0.912} (± 0.047) &  \Huge \hphantom{-}0.478 (± 0.320)  &  \Huge \hphantom{-}0.538 (± 0.317) &             \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}             &            \multicolumn{1}{c}{\Huge -}      &            \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}        \\[.3cm]
                                    
                                    \Huge Wav2vec-BERT raw avg. over time & \Huge -0.035 (± 0.434)  & \Huge \hphantom{-}0.159 (± 0.406) &  \Huge \hphantom{-}0.026 (± 0.427)  & \Huge \hphantom{-}0.105 (± 0.415) &             \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}             &            \multicolumn{1}{c}{\Huge -}      &            \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}       \\[.3cm]
                                    
                                    \Huge Wav2vec-BERT raw max. over time & \Huge  \hphantom{-}0.058 (± 0.445)  & \Huge -0.050 (± 0.441) & \Huge  \hphantom{-}0.163 (± 0.419)  & \Huge -0.150 (± 0.418) &            \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}             &            \multicolumn{1}{c}{\Huge -}      &            \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}      \\[.3cm]
                                    
                                    \Huge HuBERT raw avg. over time &  \Huge \hphantom{-}0.117 (± 0.431)  & \Huge \hphantom{-}0.109 (± 0.445) &  \Huge \hphantom{-}0.223 (± 0.448)  & \Huge \hphantom{-}0.004 (± 0.444) &             \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}             &            \multicolumn{1}{c}{\Huge -}      &            \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}    \\[.3cm]
                                    
                                    \Huge HuBERT raw max. over time &  \Huge \hphantom{-}0.026 (± 0.415)  & \Huge -0.059 (± 0.440) & \Huge -0.026 (± 0.408)  & \Huge -0.019 (± 0.441) &             \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}             &            \multicolumn{1}{c}{\Huge -}      &            \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}      \\[.3cm]
                                    
\Huge MADSpeech gender proj.  &  \Huge \hphantom{-}\textbf{0.902} (± 0.108) & \Huge \hphantom{-}\textbf{0.946} (± 0.057) &   \Huge \hphantom{-}0.708 (± 0.249)  & \Huge \hphantom{-}0.742 (± 0.216) &              \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}             &            \multicolumn{1}{c}{\Huge -}      &            \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}         \\[.3cm] \midrule[\heavyrulewidth] \\


                                  \Huge Soundstream tokens RVQ-level 0 &        \multicolumn{1}{c}{\Huge -}             &           \multicolumn{1}{c}{\Huge -}        &             \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}           & \Huge  -0.036 (± 0.452)  & \Huge \hphantom{-}0.542 (± 0.325) &    \Huge  \hphantom{-}0.237 (± 0.420)  &  \Huge \hphantom{-}0.071 (± 0.433) & \Huge  \hphantom{-}0.171 (± 0.409)  & \Huge \hphantom{-}0.002 (± 0.386) \\[.3cm]
                                  
                           \Huge Wav2vec-BERT tokens - vocab. size 256 &       \multicolumn{1}{c}{\Huge -}             &           \multicolumn{1}{c}{\Huge -}        &             \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}               & \Huge -0.192 (± 0.474)  & \Huge \hphantom{-}0.209 (± 0.438) &   \Huge   \hphantom{-}0.253 (± 0.436)  & \Huge -0.202 (± 0.415) & \Huge  \hphantom{-}0.002 (± 0.427)  & \Huge -0.103 (± 0.429) \\[.3cm]
                            
                          \Huge  Wav2vec-BERT tokens - vocab. size 512 &       \multicolumn{1}{c}{\Huge -}             &           \multicolumn{1}{c}{\Huge -}        &             \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}                & \Huge  -0.210 (± 0.423)  & \Huge \hphantom{-}0.135 (± 0.420) &   \Huge   \hphantom{-}0.262 (± 0.437)  & \Huge -0.194 (± 0.409) &  \Huge \hphantom{-}0.021 (± 0.447)  & \Huge -0.053 (± 0.438) \\[.3cm]
                          
                          \Huge Wav2vec-BERT tokens - vocab. size 1024 &     \multicolumn{1}{c}{\Huge -}             &           \multicolumn{1}{c}{\Huge -}        &             \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}              & \Huge -0.218 (± 0.430)  & \Huge \hphantom{-}0.153 (± 0.416) &   \Huge   \hphantom{-}0.262 (± 0.441)  & \Huge -0.187 (± 0.409) &  \Huge \hphantom{-}0.067 (± 0.427)  & \Huge -0.050 (± 0.440) \\[.3cm]
                          
                          \Huge Wav2vec-BERT tokens - vocab. size 4096 &    \multicolumn{1}{c}{\Huge -}             &           \multicolumn{1}{c}{\Huge -}        &             \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}               & \Huge -0.193 (± 0.433)  & \Huge \hphantom{-}0.189 (± 0.433) &   \Huge   \hphantom{-}0.265 (± 0.433)  & \Huge -0.176 (± 0.402) &  \Huge \hphantom{-}0.146 (± 0.453)  & \Huge -0.088 (± 0.444) \\[.3cm]
                             \Huge  HuBERT tokens - vocab size 50 &     \multicolumn{1}{c}{\Huge -}             &           \multicolumn{1}{c}{\Huge -}        &             \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}            & \Huge -0.374 (± 0.433)  & \Huge \hphantom{-}0.462 (± 0.316) &   \Huge   \hphantom{-}0.251 (± 0.457)  & \Huge -0.190 (± 0.417) & \Huge -0.026 (± 0.457)  & \Huge -0.007 (± 0.397) \\[.3cm]
                            \Huge  HuBERT tokens - vocab size 100 &   \multicolumn{1}{c}{\Huge -}             &           \multicolumn{1}{c}{\Huge -}        &             \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}           & \Huge -0.160 (± 0.432)  & \Huge \hphantom{-}0.350 (± 0.399) &  \Huge    \hphantom{-}0.305 (± 0.435)  & \Huge -0.280 (± 0.401) & \Huge  \hphantom{-}0.015 (± 0.450)  & \Huge -0.041 (± 0.402) \\[.3cm]
                            \Huge  HuBERT tokens - vocab size 200 &    \multicolumn{1}{c}{\Huge -}             &           \multicolumn{1}{c}{\Huge -}        &             \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}           & \Huge -0.255 (± 0.433)  & \Huge \hphantom{-}0.501 (± 0.337) &   \Huge   \hphantom{-}0.284 (± 0.451)  & \Huge -0.212 (± 0.439) &  \Huge \hphantom{-}0.069 (± 0.423)  & \Huge -0.064 (± 0.447) \\[.3cm]
\bottomrule[\heavyrulewidth] \\ \toprule[\heavyrulewidth] \\






                                                 \multicolumn{11}{c}{\Huge Speaker voices}  \\[.2cm] \midrule[\heavyrulewidth] \\
  &     \multicolumn{2}{c}{\Huge Avg. Cosine}                  &        \multicolumn{2}{c}{\Huge Vendi score} & \multicolumn{2}{c}{\Huge Token entropy}                  & \multicolumn{2}{c}{\Huge Distinct n-grams} & \multicolumn{2}{c}{\Huge self-BLEU} \\[.2cm] \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \\
                                                   
                                                 &         \Huge      Male &    \Huge       Female &       \Huge        Male &      \Huge     Female &       \Huge\Huge        Male &      \Huge    Female &         \Huge         Male &     \Huge      Female &       \Huge        Male &        \Huge   Female \\[.2cm] \midrule[\heavyrulewidth] \\
  
\Huge Soundstream raw avg. over time & \Huge \hphantom{-}0.544 (± 0.312) & \Huge \hphantom{-}0.234 (± 0.426) & \Huge \hphantom{-}0.759 (± 0.175) &  \Huge \hphantom{-}0.731 (± 0.284) &     \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}             &            \multicolumn{1}{c}{\Huge -}      &            \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}          \\[.3cm]

\Huge Soundstream raw max. over time & \Huge -0.611 (± 0.060) & \Huge -0.598 (± 0.082) & \Huge -0.903 (± 0.095) & \Huge -0.750 (± 0.215) &    \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}             &            \multicolumn{1}{c}{\Huge -}      &            \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}           \\[.3cm]
                                 
\Huge Speech Sim & \Huge \hphantom{-}0.811 (± 0.074) & \Huge \hphantom{-}0.834 (± 0.073) & \Huge \hphantom{-}\textbf{1.000} (± 0.000) & \Huge \hphantom{-}\textbf{1.000} (± 0.000) &  \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}             &            \multicolumn{1}{c}{\Huge -}      &            \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}            \\[.3cm]
                                      
\Huge Trained from scratch & \Huge \hphantom{-}0.480 (± 0.200) & \Huge \hphantom{-}0.666 (± 0.200) & \Huge \hphantom{-}0.962 (± 0.044) & \Huge \hphantom{-}\underline{0.963} (± 0.053) &     \multicolumn{1}{c}{\Huge -}         &          \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}             &            \multicolumn{1}{c}{\Huge -}      &            \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}           \\[.3cm]

\Huge Wav2vec-BERT raw avg. over time & \Huge -0.448 (± 0.194) & \Huge -0.118 (± 0.258) & \Huge -0.419 (± 0.193) & \Huge -0.094 (± 0.245) &  \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}             &            \multicolumn{1}{c}{\Huge -}      &            \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}             \\[.3cm]

\Huge Wav2vec-BERT raw max. over time & \Huge -0.618 (± 0.045) & \Huge -0.430 (± 0.249) & \Huge -0.643 (± 0.027) & \Huge -0.520 (± 0.193) &  \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}             &            \multicolumn{1}{c}{\Huge -}      &            \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}            \\[.3cm]

\Huge HuBERT raw avg. over time & \Huge \Huge -0.575 (± 0.094) & \Huge -0.178 (± 0.291) & \Huge -0.447 (± 0.202) &  \Huge \hphantom{-}0.007 (± 0.321) &   \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}             &            \multicolumn{1}{c}{\Huge -}      &            \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}             \\[.3cm]

\Huge HuBERT raw max. over time  & \Huge -0.639 (± 0.045) & \Huge -0.471 (± 0.242) & \Huge -0.642 (± 0.028) & \Huge -0.424 (± 0.275) &   \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}             &            \multicolumn{1}{c}{\Huge -}      &            \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}              \\ [.3cm]

\Huge MADSpeech speaker voice proj. & \Huge \hphantom{-}0.823 (± 0.063) & \Huge \hphantom{-}0.881 (± 0.077) & \Huge \Huge \hphantom{-}\underline{0.993} (± 0.019) & \Huge \hphantom{-}\textbf{1.000} (± 0.000) &    \multicolumn{1}{c}{\Huge -}         &           \multicolumn{1}{c}{\Huge -}      &          \multicolumn{1}{c}{\Huge -}             &            \multicolumn{1}{c}{\Huge -}      &            \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}              \\[.3cm] \midrule[\heavyrulewidth] \\


\Huge Soundstream tokens RVQ-level 0 &   \multicolumn{1}{c}{\Huge -}             &           \multicolumn{1}{c}{\Huge -}        &             \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}           & \Huge \hphantom{-}0.977 (± 0.044) & \Huge \Huge\hphantom{-}0.928 (± 0.100) &  \Huge \hphantom{-}0.515 (± 0.258) &  \Huge -0.077 (± 0.489) & \Huge \hphantom{-}0.494 (± 0.296) & \Huge -0.027 (± 0.593) \\[.3cm]

\Huge Wav2vec-BERT tokens - vocab. size 256 &    \multicolumn{1}{c}{\Huge -}             &           \multicolumn{1}{c}{\Huge -}        &             \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}             & \Huge \hphantom{-}0.951 (± 0.067) & \Huge \Huge\hphantom{-}0.745 (± 0.289) &   \Huge   -0.904 (± 0.151) & \Huge -0.893 (± 0.151) & \Huge -0.917 (± 0.107) & \Huge -0.815 (± 0.235) \\[.3cm]

\Huge Wav2vec-BERT tokens - vocab. size 512 &  \multicolumn{1}{c}{\Huge -}             &           \multicolumn{1}{c}{\Huge -}        &             \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}            & \Huge \hphantom{-}0.968 (± 0.062) & \Huge \hphantom{-}0.911 (± 0.116) &    \Huge  -0.870 (± 0.178) & \Huge -0.787 (± 0.274) & \Huge -0.898 (± 0.099) & \Huge -0.722 (± 0.348) \\[.3cm]
                           
\Huge Wav2vec-BERT tokens - vocab. size 1024 &   \multicolumn{1}{c}{\Huge -}             &           \multicolumn{1}{c}{\Huge -}        &             \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}             & \Huge \hphantom{-}0.976 (± 0.049) & \Huge \hphantom{-}0.923 (± 0.105) &    \Huge  -0.870 (± 0.168) & \Huge -0.699 (± 0.327) & \Huge -0.893 (± 0.115) & \Huge -0.768 (± 0.246) \\[.3cm]

\Huge Wav2vec-BERT tokens - vocab. size 4096 &  \multicolumn{1}{c}{\Huge -}             &           \multicolumn{1}{c}{\Huge -}        &             \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}             & \Huge \hphantom{-}0.979 (± 0.044) & \Huge \hphantom{-}0.928 (± 0.099) &    \Huge  -0.736 (± 0.272) & \Huge -0.266 (± 0.526) & \Huge -0.919 (± 0.085) & \Huge -0.645 (± 0.394) \\[.3cm]

\Huge HuBERT tokens - vocab size 50 &   \multicolumn{1}{c}{\Huge -}             &           \multicolumn{1}{c}{\Huge -}        &             \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}             & \Huge \hphantom{-}0.949 (± 0.075) & \Huge \hphantom{-}0.907 (± 0.130) &   \Huge   -0.965 (± 0.067) & \Huge -0.888 (± 0.134) & \Huge -0.213 (± 0.468) & \Huge -0.118 (± 0.567) \\[.3cm]
                              
\Huge HuBERT tokens - vocab size 100 &   \multicolumn{1}{c}{\Huge -}             &           \multicolumn{1}{c}{\Huge -}        &             \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}            & \Huge \hphantom{-}0.766 (± 0.222) & \Huge \hphantom{-}0.862 (± 0.171) &   \Huge   -0.966 (± 0.068) & \Huge -0.869 (± 0.174) & \Huge -0.658 (± 0.286) & \Huge -0.442 (± 0.503) \\[.3cm]
                              
\Huge HuBERT tokens - vocab size 200 &  \multicolumn{1}{c}{\Huge -}             &           \multicolumn{1}{c}{\Huge -}        &             \multicolumn{1}{c}{\Huge -}        &        \multicolumn{1}{c}{\Huge -}           & \Huge \hphantom{-}0.874 (± 0.158) & \Huge \hphantom{-}0.877 (± 0.145) &    \Huge  -0.963 (± 0.068) & \Huge -0.839 (± 0.195) & \Huge -0.872 (± 0.117) & \Huge  -0.557 (± 0.450) \\[.3cm] \bottomrule[\heavyrulewidth] 
\end{tabular}}
\caption{Results for gender and speaker voices experiments. Average spearman correlations (and standard errors) between the variation of gender (resp. number of different speaker voices) and different combination of speech representations and metrics. Best results are highlighted in bold, second best results are underlined.}
\label{tab:gender-speakers-tab}
\end{table*}


==> tables/speakers_control_gender.tex <==
\begin{table}[!h]
\centering
\resizebox{\linewidth}{!}{\begin{tabular}{lcc}
\toprule

&    Avg. cosine               &       Vendi score  \\ \midrule

SpeechSim & 0.720 (± 0.196)  &  \textbf{0.995} (± 0.016)     \\

From scratch &  -0.216 (± 0.288)  &  0.421 (± 0.207)    \\

MADSpeech/Speaker & 0.583 (± 0.232)  &  \underline{0.926} (± 0.085)  \\ 
\bottomrule
\end{tabular}}
\caption{Spearman correlation of diversity measures with the speaker diversity while the gender proportion in the samples is varied from uniform to single-gender. Best results are in bold, second best results are underlined.}
\label{tab:speakers_control_gender_tab}
\end{table}


==> tables/zero-shot-emotions.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcc}
\toprule
& \multicolumn{2}{c}{EmoV} \\
&    Avg. cosine               &       Vendi score  \\ 
\midrule
Speech Sim & 0.809 (± 0.200)  &  0.823 (± 0.193)     \\
Trained from scratch on Expresso only &  0.498 (± 0.250)  &  0.513 (± 0.274)    \\
SpeechSim/Emotion-Expresso  & 0.641 (± 0.279)  &  0.709 (± 0.243)  \\
\midrule
& \multicolumn{2}{c}{Expresso} \\ 
&    Avg. cosine               &       Vendi score  \\
\midrule
Speech Sim & 0.739 (± 0.249) &  0.864 (± 0.128)     \\
Trained from scratch/EmoV &   0.247 (± 0.562)  &  0.251 (± 0.512)  \\
SpeechSim/Emotion-EmoV & 0.273 (± 0.465) & 0.321 (± 0.464)  \\
\bottomrule
\end{tabular}
}
\caption{Average Spearman correlations ($\pm$ standard error) between the classes entropy in EmoV and Expresso samples and diversity scores induced by speech representations.}
\label{tab:zero-shot-emotion}
\end{table}

